SubGDiff: A Subgraph Diffusion Model to Improve Molecular Representation Learning

Molecular representation learning has shown great success in advancing AI-based drug discovery. The core of many recent works is based on the fact that the 3D geometric structure of molecules provides essential information about their physical and chemical characteristics. Recently, denoising diffusion probabilistic models have achieved impressive performance in 3D molecular representation learning. However, most existing molecular diffusion models treat each atom as an independent entity, overlooking the dependency among atoms within the molecular substructures. This paper introduces a novel approach that enhances molecular representation learning by incorporating substructural information within the diffusion process. We propose a novel diffusion model termed SubGDiff for involving the molecular subgraph information in diffusion. Specifically, SubGDiff adopts three vital techniques: i) subgraph prediction, ii) expectation state, and iii) k-step same subgraph diffusion, to enhance the perception of molecular substructure in the denoising network. Experimentally, extensive downstream tasks demonstrate the superior performance of our approach. The code is available at https://github.com/youjibiying/SubGDiff.

==> 7_2_lemma.tex <==
\subsection{An important lemma for diffusion model}
\vspace{-2mm}
According to \citep{sohl2015deep, ho2020denoising}, the diffusion model is trained by optimizing the variational bound on the negative log-likelihood $-\log p_{\theta}(R^0)$, in which the tricky terms are $L_{t-1}=D_{KL}(q(R^{t-1}| R^t, R^0) || p_{\theta}(R^{t-1}| R^t)))$, $T\geq t>1$. 
Here we provide a lemma that tells us the posterior distribution $q(R^{t-1}| R^t, R^0)$ used in the training and sampling algorithms of the diffusion model can be determined by $q(R^t|R^{t-1}, R^0)$, $q(R^{t-1}|R^0)$. Formally, we have
\begin{snugshade}
\vspace{-.2cm}

\begin{restatable}[]{lemma}{restalemmtwo}
    \label{Lemma:diffusion}
    Assume the forward and reverse processes of the diffusion model are both Markov chains.
Given the forward Gaussian distribution $q(R^t|R^{t-1},R^0) = \mcal N(R^t; \mu_1 R^{t-1},\sigma_1^2 \textbf{I})$, $q(R^{t-1}|R^0) = \mcal N(R^{t-1}; \mu_2R^0,\sigma_2^2 \textbf{I})$ and $\epsilon_0 \sim \mcal N(\mbf 0, \mbf I)$, the distribution $q(R^{t-1}|R^t,R^0)$ is 
\vspace{-1mm}
\begin{align*}
\scalemath{0.8}{q(R^{t-1}|R^t,R^0)\propto\mcal N(R^{t-1}; \frac{1}{\mu_1}(R^t - \frac{\sigma_1^2}{\sqrt{\mu_1^2\sigma_2^2 + \sigma_1^2}}\epsilon_0 ), \frac{\sigma_1^2 \sigma_2^2 }{\mu_1^2 \sigma_2^2 + \sigma_1^2}\textbf{I}) }.
\end{align*}

Parameterizing $p_\theta(R^{t-1}|R^t)$ in the reverse process as $\mcal N(R^{t-1}; \frac{1}{\mu_1}(R^t - \frac{\sigma_1^2}{\sqrt{\mu_1^2\sigma_2^2 + \sigma_1^2}}\epsilon_\theta(R^t,t) ), \frac{\sigma_1^2 \sigma_2^2 }{\mu_1^2 \sigma_2^2 + \sigma_1^2}\textbf{I})$ 
, the training objective of the DPM can be written as
\vspace{-2mm}
\begin{align*}
    \scalemath{0.84}{\mcal L(\theta) =  \mbb E_{t,R^0, 
    \epsilon}\Big[ \frac{\sigma_1^2}{2\mu_1^2\sigma_2^2} \|\epsilon-\epsilon_{\theta }(\mu_1\mu_2 R^0 + \sqrt{\mu_1^2\sigma_2^2 + \sigma_1^2}\epsilon, t)\|^2\Big]},
\end{align*}
and the sampling (reverse) process is 
\vspace{-3mm}
\begin{align}
\label{eq:sampling_diffusion}
    \scalemath{0.8}{R^{t-1} = \frac{1}{\mu_1}\left(R^t - \frac{\sigma_1^2}{\sqrt{\mu_1^2\sigma_2^2 + \sigma_1^2}}\epsilon_{\theta}(R^t,t)\right) +  \frac{\sigma_1 \sigma_2 }{\sqrt{\mu_1^2 \sigma_2^2 + \sigma_1^2}} z ,}
\end{align}
where $ z\sim \mcal N(\mbf 0, \mbf I)$.
\end{restatable}
\vspace{-.1cm}
\end{snugshade}
The proof of the lemma can be found in the Appendix.
Once we get the variables $(\mu_1,\sigma_1,\mu_2,\sigma_2)$, we can directly obtain the training objective and sampling process via lemma \ref{Lemma:diffusion}, which will help the design of new diffusion models.



\vspace{-2mm}

==> figures/fig_dynamic_mask_diff.tex <==
\begin{figure*}
    \centering
    % \vspace{-1cm}
    \includegraphics[width=1\linewidth]{figures/dynamic_mask.pdf}
     \caption{An example of dynamic mask diffusion}
    \label{fig:dynamic_mask_diff}
        % \vspace{-4mm}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}


% ===============================add by jiying==========================================

\newcommand{\todo}[1]{\textcolor{magenta}{(TODO:#1)}} %magenta
% \newcommand{\todo}[1]{\textcolor{magenta}{}} %magenta
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}

\newcommand{\mcal}[1]{\mathcal{#1}}


% =========================================================================

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\s{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\R{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


% ### add by jiying----------------------

\newcommand{\lowbound}[1]{\lfloor{#1}\rfloor}

==> tables/tab_comformation_generation_SOTA.tex <==

\begin{table}[!t]
    % \vspace{-10pt}
    \centering
    \caption{Results on the \textbf{GEOM-Drugs} dataset. The threshold $\delta=1.25\si{\angstrom}$}
    \label{tab:drugs}
    % \hspace{-0.4cm}
    \resizebox{\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lc|cccc|cccc}
    \toprule[1.0pt]
    & &  \multicolumn{2}{c}{\shortstack[c]{COV-R (\%) $\uparrow$}} & \multicolumn{2}{c|}{\shortstack[c]{MAT-R (\si{\angstrom}) $\downarrow$ }}  & \multicolumn{2}{c}{\shortstack[c]{COV-P (\%) $\uparrow$}}  & \multicolumn{2}{c}{\shortstack[c]{MAT-P (\si{\angstrom}) $\downarrow$ }} \\
    % \cline{2-9}
     Models& Sampling method & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\
    % \hline \hline
    \midrule[0.8pt]
    \CVGAE & -& 0.00 & 0.00 & 3.0702 & 2.9937 & - & - & - & - \\ 
    \GraphDG & -& 8.27 & 0.00 & 1.9722 & 1.9845 & 2.08 & 0.00 & 2.4340 & 2.4100 \\ 
    \CGCF & -& 53.96 & 57.06 & 1.2487 & 1.2247 & 21.68 & 13.72 & 1.8571 & 1.8066 \\
    \ConfVAE & -& 55.20 & 59.43 & 1.2380 & 1.1417 & 22.96 & 14.05 & 1.8287 & 1.8159 \\
    \GeoMol & -& 67.16 & 71.71 & 1.0875 & 1.0586 & - & - & - & - \\ 
    \ConfGF &Langevin dynamics & 62.15 & 70.93 & 1.1629 & 1.1596 & 23.42 & 15.52 & 1.7219 & 1.6863 \\
   {\GeoDiff} & DDPM &    56.31 &  57.73 & 1.2159 &  1.2053 &  56.44 & 61.62 & 1.3309 & 1.1781 \\
{\GeoDiff} & Langevin dynamics &  \bf 89.13 & \bf 97.88 & \bf 0.8629 & \bf 0.8529 & \bf 61.47 & \bf 64.55 & \bf 1.1712 & \bf 1.1232 \\
    \midrule[0.3pt]
    \bf \method &Langevin dynamics & 87.67 &  97.30 &  0.8978 &  0.8938 & 57.40 &  57.08 &  3.5724 &  1.2438 \\
    \bf \method & DDPM & 87.86 &  96.71 &  0.9038 &  0.8984 & 54.38 &  54.03&  2.2250 &  1.2456 \\
    \bottomrule[1.0pt]
    \end{tabular}
    \end{threeparttable}
    }
\end{table}

% \subsection{Results for GEOM-QM9}



==> tables/tab_comformation_generation_drug_8metrics.tex <==


\begin{table}[!t]
    \vspace{-18pt}
     \caption{\revise{Results on the \textbf{GEOM-Drugs} dataset under different diffusion timesteps. DDPM~\citep{ho2020denoising} is the sampling method used in GeoDiff. Our proposed sampling method (Algorithm \ref{alg:SamplingSubGDiff}) can be viewed as a DDPM variant. \up/\down denotes  \method outperforms/underperforms  \GeoDiff.
    % without FF optimization. 
    The threshold $\delta=1.25\si{\angstrom}$}.}
    \label{tab:qm9}
     \vspace{-9.5pt}
    % \hspace{-0.4cm}
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{lcl|llll|llll}
    \toprule[1.0pt]
     & & & \multicolumn{2}{c}{\shortstack[c]{COV-R (\%) $\uparrow$}} & \multicolumn{2}{c|}{\shortstack[c]{MAT-R (\si{\angstrom}) $\downarrow$ }}  & \multicolumn{2}{c}{\shortstack[c]{COV-P (\%) $\uparrow$}}  & \multicolumn{2}{c}{\shortstack[c]{MAT-P (\si{\angstrom}) $\downarrow$ }} \\
    % \cline{2-9}
     Models & Timesteps& Sampling method &  Mean & Median & Mean & Median & Mean & Median & Mean & Median \\
    \midrule[0.8pt]
        \GeoDiff&   500& DDPM &  50.25   &   48.18& 1.3101& 1.2967 & 53.41   &   61.81 & 1.4075 & 1.1980 \\
        \method& 500&  DDPM (ours) &  {76.16}\up	& {86.43}\up	&{1.0463}\up	&{1.0264}\up&	\up&	\up	&\up	&{}\up\\
                 \midrule[0.3pt]
 \GeoDiff&  500& LD  &     64.12    &   75.56& 1.1444 & 1.1246  & 29.22 &     21.03 & 1.5654 & 1.5255 \\
 
\method &  200& LD (ours) &       74.30\up   &    77.87\up & 1.0003\up & 0.9905\up & 66.06\up  &    74.26\up  & 1.3250\up & 1.1487\up \\
    \bottomrule[1.0pt]
    \end{tabular}
    }
    \vspace{-0.48cm}. 
\end{table}


==> tables/tab_comformation_generation_full.tex <==


\begin{table}[!t]
    \vspace{-15pt}
     \caption{Results on \textbf{GEOM-QM9} dataset. Langevin dynamics~\citep{song2019generative} and DDPM~\citep{ho2020denoising} are two different sampling techniques in DPM.
    % without FF optimization. 
    The threshold $\delta=0.5\si{\angstrom}$.}
    \label{tab:qm9_full}
     \vspace{-10pt}
    % \hspace{-0.4cm}
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{llc|llll|llll}
    \toprule[1.0pt]
     & & & \multicolumn{2}{c}{\shortstack[c]{COV-R (\%) $\uparrow$}} & \multicolumn{2}{c|}{\shortstack[c]{MAT-R (\si{\angstrom}) $\downarrow$ }}  & \multicolumn{2}{c}{\shortstack[c]{COV-P (\%) $\uparrow$}}  & \multicolumn{2}{c}{\shortstack[c]{MAT-P (\si{\angstrom}) $\downarrow$ }} \\
    % \cline{2-9}
    Steps& Sampling method &  Models & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\
    \midrule[0.8pt]
     5000&  Langevin dynamics& \GeoDiff&  88.35 & 92.55
 & \bf 0.2166
 & \bf 0.2154  &  \underline{52.67}  &  \underline{50.00} & \bf 0.4398 & 0.4264 \\
    5000&Langevin dynamics &\bf \method &  \underline{88.76}$\uparrow$ & \underline{94.23}$\uparrow$ & \underline{0.2343}$\downarrow$  & \underline{0.2244}$\downarrow$  & 50.28$\downarrow$  & 49.62$\downarrow$ & \underline{0.4728}$\downarrow$  & 0.4549$\downarrow$ \\
    
    \midrule[0.3pt]
          5000& DDPM & \GeoDiff&   80.36 & 83.82 
 &  0.2820 & 0.2799   & \bf 53.66 & \bf 50.85  & 0.6673   & \bf 0.4214 \\
      
        5000&  DDPM &\bf \method & \textbf{90.91}$\downarrow$  & \textbf{95.59}$\uparrow$ & {0.2460}$\downarrow$ & {0.2351}$\uparrow$ & 50.16$\downarrow$ & 48.01$\downarrow$ & 0.6114$\uparrow$ & 0.4791$\downarrow$\\
    \midrule[0.5pt]
          500& DDPM & \GeoDiff&  80.20   &   83.59& 0.3617& 0.3412 & 45.4893    &  45.45 & 1.1518  &0.5087  \\
        500&  DDPM &\bf \method& 86.61$\uparrow$	& 90.26$\uparrow$	&0.2693$\uparrow$	&0.2577$\uparrow$&	51.25$\uparrow$&	48.76$\uparrow$	&0.6862$\uparrow$	&0.4621$\uparrow$\\
                 \midrule[0.3pt]
       500&Langevin dynamics &\GeoDiff & 87.80	&93.66&	0.3179	&0.3216	&46.25&	45.02&	0.6173	&0.5112 \\
       500&Langevin dynamics &\bf \method & 91.40$\uparrow_{3.6}$    &  95.39$\uparrow_{1.73}$  &  0.2543$\uparrow_{0.0636}$  & 0.2601$\uparrow_{0.0615}$ & 51.71$\uparrow_{5.46}$  &   48.50$\uparrow_{3.48}$& 0.5035$\uparrow_{0.1138}$ & 0.4734$\uparrow_{0.0378}$ \\
\midrule[0.5pt]
200& Langevin dynamics & \GeoDiff&       86.60   &   93.09 & 0.3532 & 0.3574 & 42.98     &  42.60 & 0.5563 & 0.5367 \\
200& Langevin dynamics & \method &       90.36$\uparrow$   &   95.93$\uparrow$ &  0.3064$\uparrow$ & 0.3098$\uparrow$ & 48.56$\uparrow$  &    46.46$\uparrow$  & 0.5540$\uparrow$ & 0.5082$\uparrow$ \\
200& DDPM  & \GeoDiff&      69.90    &   72.04& 0.4222 & 0.4272 & 36.71 &     33.51 & 0.8532 & 0.5554 \\
200& DDPM & \method &      85.53$\uparrow$   &    88.99$\uparrow$ &  0.2994$\uparrow$ & 0.3033$\uparrow$ & 47.76$\uparrow$  &    45.89$\uparrow$  & 0.6971$\uparrow$ & 0.5118$\uparrow$ \\
    \bottomrule[1.0pt]
    \end{tabular}
    }
    \vspace{-0.3cm}. 
\end{table}









































% \begin{table*}[thbp]
% \def\p{$\pm$} 
% \centering
% \setlength\tabcolsep{5pt} %调整列宽
% % \vspace{-2mm}
% \caption{Results on 12 quantum mechanics prediction tasks from QM9. We take 110K for training, 10K for validation, and 11K for testing. The evaluation is mean absolute error~(MAE), and the best and the second best results are marked in bold and bold, respectively. }
%     % \vspace{-2mm}
% \scalebox{0.99}{
% \begin{tabular}{ccccc|cccc}
% \toprule
% \multirow{1}{*}{} & \multicolumn{2}{c}{COV-R (\%)$\uparrow$ } & \multicolumn{2}{c}{MAT-R (\%)$\downarrow$} & \multicolumn{2}{c}{COV-P (\%)$\uparrow$} & \multicolumn{2}{c|}{MAT-P (\%)$\downarrow$} \\
% % \cline{2-9}
%  % & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
%  Models & Mean & Median& Mean & Median & Mean & Median & Mean & Median \\
% \midrule
% CVGAE & & & & & & & & \\
% GRAPHDG & & & & & & & & \\
% CGCF & & & & & & & & \\
% CONFCAE & & & & & & & & \\
% GEO & & & & & & & & \\
% \bottomrule
% \end{tabular}
% }
%     \vspace{-2mm}
%     \label{tab:object_accuracy} 
% \end{table*}

==> tables/tab_domain_generalization.tex <==


\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.50\textwidth}
\makeatletter\def\@captype{table}
\tiny
    \begin{tabular}{lc|cccc}
    \toprule[1.0pt]
     & & \multicolumn{2}{c}{\shortstack[c]{COV-R (\%) $\uparrow$}} & \multicolumn{2}{c|}{\shortstack[c]{MAT-R (\si{\angstrom}) $\downarrow$ }}   \\
 
    Models &  Training data & Mean & Median & Mean & Median  \\
    \midrule[0.8pt]
    \CVGAE & GEOM-QM9 & 0.09 & 0.00 & 1.6713 & 1.6088  \\ 
    \GraphDG & GEOM-QM9 &  73.33 & 84.21 & 0.4245 & 0.3973 \\ 
    \CGCF & GEOM-QM9 & 78.05 & 82.48 & 0.4219 & 0.3900  \\
    \ConfVAE & GEOM-QM9 & 77.84 & 88.20 & 0.4154 & 0.3739  \\
    \GeoMol & GEOM-QM9 & 71.26 & 72.00 & 0.3731 & 0.3731 \\ 

     \GeoDiff&  GEOM-Drugs& 74.94 & 79.15 &  0.3492 &  0.3392   \\

      \midrule[0.3pt]
    \bf \method &  GEOM-Drugs &\textbf{83.50} & \textbf{88.70} & \bf{0.3116} & \bf{0.3075} \\

    \bottomrule[1.0pt]
    \end{tabular}  
\caption{Results on the \textbf{GEOM-QM9} dataset. The threshold $\delta=0.5\si{\angstrom}$}
%     \label{tab:qm9_DG}
\end{minipage}
\begin{minipage}[t]{0.50\textwidth}
\makeatletter\def\@captype{table}
\tiny
    \begin{tabular}{lc|cccc}
    \toprule[1.0pt]
     & & \multicolumn{2}{c}{\shortstack[c]{COV-R (\%) $\uparrow$}} & \multicolumn{2}{c|}{\shortstack[c]{MAT-R (\si{\angstrom}) $\downarrow$ }}   \\
    % \cline{2-9}
    Models &  Training data & Mean & Median & Mean & Median  \\
    \midrule[0.8pt]
    \CVGAE & GEOM-Drugs & 0.00 & 0.00 & 3.0702 & 2.9937  \\ 
    \GraphDG & GEOM-Drugs &  8.27 & 0.00 & 1.9722& 1.9845 \\ 
 \GeoDiff&  GEOM-QM9& 7.99
 & 0.00 &  2.7704 &  2.3297   \\
      \midrule[0.3pt]
    \bf \method &  GEOM-QM9 &\textbf{24.01} & \textbf{9.93} & \bf{1.6128} & \bf{1.5819} \\
    \bottomrule[1.0pt]
    \end{tabular}
     \caption{Results on the \textbf{GEOM-Drugs} dataset. The threshold $\delta=1.25\si{\angstrom}$}

\end{minipage}
\end{minipage}


==> tables/tab_moleculesde_3d.tex <==
\begin{table*}[htb]
\setlength{\tabcolsep}{5pt}
\fontsize{9}{9}\selectfont
\caption{
\small
Results on 12 quantum mechanics prediction tasks from QM9. We take 110K for training, 10K for validation, and 11K for testing. The evaluation is mean absolute error, and the best and the second best results are marked in \underline{\textbf{bold}} and \textbf{bold}, respectively.
}
% \vspace{-2ex}
\label{tab:main_QM9_result}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c c c c c c}
\toprule

Pretraining & $\alpha$ $\downarrow$ & $\nabla \mathcal{E}$ $\downarrow$ & $\mathcal{E}_\text{HOMO}$ $\downarrow$ & $\mathcal{E}_\text{LUMO}$ $\downarrow$ & $\mu$ $\downarrow$ & $C_v$ $\downarrow$ & $G$ $\downarrow$ & $H$ $\downarrow$ & $R^2$ $\downarrow$ & $U$ $\downarrow$ & $U_0$ $\downarrow$ & ZPVE $\downarrow$\\
\midrule

% 5e-4_CosineAnnealingLR_300_128_1000
-- (random init) & 0.060 & 44.13 & 27.64 & 22.55 & 0.028 & 0.031 & 14.19 & 14.05 & 0.133 & 13.93 & 13.27 & 1.749\\



Type Prediction & 0.073 & 45.38 & 28.76 & 24.83 & 0.036 & 0.032 & 16.66 & 16.28 & 0.275 & 15.56 & 14.66 & 2.094\\

Distance Prediction & 0.065 & 45.87 & 27.61 & 23.34 & 0.031 & 0.033 & 14.83 & 15.81 & 0.248 & 15.07 & 15.01 & 1.837\\

% pretrain_TorsionAnglePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_1e-3_100
Angle Prediction & 0.066 & 48.45 & 29.02 & 24.40 & 0.034 & 0.031 & 14.13 & 13.77 & 0.214 & 13.50 & 13.47 & 1.861\\

% pretrain_3DInfoGraph/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
3D InfoGraph & 0.062 & 45.96 & 29.29 & 24.60 & 0.028 & 0.030 & 13.93 & 13.97 & 0.133 & 13.55 & 13.47 & 1.644\\

RR & 0.060 & 43.71 & 27.71 & 22.84 & 0.028 & 0.031 & 14.54 & 13.70 & \textbf{0.122} & 13.81 & 13.75 & 1.694\\


InfoNCE & 0.061 & 44.38 & 27.67 & 22.85 & \textbf{0.027} & 0.030 & 13.38 & 13.36 & \underline{\textbf{0.116}} & 13.05 & 13.00 & 1.643\\


EBM-NCE & 0.057 & 43.75 & 27.05 & 22.75 & 0.028 & 0.030 & 12.87 & 12.65 & 0.123 & 13.44 & 12.64 & 1.652\\


3D InfoMax & 0.057 & 42.09 & 25.90 & 21.60 & 0.028 & 0.030 & 13.73 & 13.62 & 0.141 & 13.81 & 13.30 & 1.670\\

% pretrain_GraphMVP/PCQM4Mv2_schnet/Vanilla_1e-4_0.3_100
GraphMVP & 0.056 & 41.99 & 25.75 & \textbf{21.58} & \textbf{0.027} & \textbf{0.029} & 13.43 & 13.31 & 0.136 & 13.03 & 13.07 & 1.609\\


 % pretrain_DeepMind/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.15_GeoSSL_10_0.01_30_symmetry_0.1_100
Denoising & 0.058 & 42.64 & 26.32 & 21.87 & 0.028 & 0.030 & 12.61 & 12.81 & 0.173 & 12.45 & 12.12 & 1.696\\

% pretrain_GeoSSL/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0_GeoSSL_10_0.01_30_symmetry_0.05_100
GeoSSL & 0.056 & 42.29 & \underline{\textbf{25.61}} & 21.88 & \textbf{0.027} & \textbf{0.029} & \textbf{11.54} & \textbf{11.14} & 0.168 & \textbf{11.06} & \underline{\textbf{10.96}} & 1.660\\

\midrule


MoleculeSDE (VE) & \textbf{0.056} & \textbf{41.84} & 25.79 & 21.63 & \textbf{0.027} & \textbf{0.029} & \underline{\textbf{11.47}} & \underline{\textbf{10.71}} & 0.233 & \underline{\textbf{11.04}} & \textbf{10.95} & \underline{\textbf{1.474}}\\

MoleculeSDE (VP) & \underline{\textbf{0.054}} & \underline{\textbf{41.77}} & \textbf{25.74} & \underline{\textbf{21.41}} & \underline{\textbf{0.026}} & \underline{\textbf{0.028}} & 13.07 & 12.05 & 0.151 & 12.54 & 12.04 & \textbf{1.587}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-2ex}
\end{table*}

